Efficient State-based CRDTs by Delta-Mutation

CRDTs are distributed data types that make eventual consistency of a distributed object possible and non ad-hoc. Specifically, state-based CRDTs ensure convergence through disseminating the en- tire state, that may be large, and merging it to other replicas; whereas operation-based CRDTs disseminate operations (i.e., small states) assuming an exactly-once reliable dissemination layer. We introduce Delta State Conflict-Free Replicated Datatypes ({\delta}-CRDT) that can achieve the best of both worlds: small messages with an incremental nature, as in operation-based CRDTs, disseminated over unreliable communication channels, as in traditional state-based CRDTs. This is achieved by defining {\delta}-mutators to return a delta-state, typically with a much smaller size than the full state, that is joined to both: local and remote states. We introduce the {\delta}-CRDT framework, and we explain it through establishing a correspondence to current state-based CRDTs. In addition, we present an anti-entropy algorithm that ensures causal consistency, and we introduce two {\delta}-CRDT specifications of well-known replicated datatypes.

==> design.tex <==
\section{Delta State Replicated Data Types: $\dsrdt$}
\label{sec:model}
In this section, we introduce a new approach to design efficient state-based CRDTs. We start with some definitions and then we explore the correctness of the approach showing how it can be used to improve the performance of state-based CRDTs. The following definition introduces \dsrdt.

\subsection{Definitions}
\label{subs:dsrdt}

\begin{definition}[\dsrdt]
\label{def:dsrdt}
A \dsrdt is a state-based CRDT D=(S,M,Q) where for each mutator $m\in M$ there exist a corresponding delta-mutator $m^\delta \in M$ such that for a given replica i with any state $X_i\in S$, \[m(X_i)=X_i\sqcup m^\delta(X_i) .\]
\end{definition}

The above definition is a relaxed version of that of state-based CRDTs (defined in~\cite{tech report}). In fact, in any state-based CRDT, any mutator $m\in M$ is a delta-mutator itself since $m(X_i)=X_i\sqcup m(X_i)$ ($\sqcup$ is idempotent). However, the above definition allows for, possibly, a range of $\delta$-mutators which can lead to performance improvements as we investigate later. We call a $\delta$-mutator $m^\delta$ corresponding to $m\in M$ with the property $m(X_i)=m^\delta(X_i)$ a \emph{maximal} mutator. On the other hand, a $\delta$-mutator $m^\delta$ is said to be \emph{minimal} if for every $\delta$-mutator $m'^\delta$ corresponding to $m\in M$,  $size(m'^\delta(X_i))\geq size(m^\delta(X_i))~\forall i$.

\subsection{State Transition in \dsrdt}
\label{subs:transition}
Def.~\ref{def:dsrdt} defines the basic method for state transition in \dsrdt: a state $X'=X\sqcup \dm(X)$ is a transition from state $X$ to $X'$ through applying the $\delta$-mutator $\dm$. Interestingly, since applying operations in \dsrdt is as simple as joining a delta to the original state, then state transition can be batched in such a way that multiple operations are subsequently applied before getting merged to the original replica state. This is very useful to achieve convergence across different replicas by only shipping deltas (or groups of deltas), produced by $\delta$-mutators, to be joined by the remote replica. To ensure correctness, we introduce the following proposition.

\begin{proposition}[Delta-groups of \dsrdt]
Consider a \dsrdt D=(S,M,Q), and a replica $X\in D$ with state $X^0\in S$. Subsequently applying any number m of $\delta$-mutators $\dm_1,\dm_2, ..., \dm_m$ on $X^0$, is equivalent to 'joining' all the corresponding deltas $\delta^1,\delta^2, ..., \delta^m$, respectively, to $X^0$: 
\begin{equation}
\label{eq:hyp_groups}
X^m=\dm_m o~\dm_{m-1}~o ... o~\dm_1(X^0)=X^0\sqcup \delta^1\sqcup \delta^2 \sqcup ... \sqcup \delta^m.
\end{equation}

\end{proposition}
\begin{proof}
We prove this by induction in two steps: (1) proving that the above hypothesis is true for m=1, and (2) if the hypothesis is true for m-1, then it is true for m.

For m=1, i.e., applying only one mutator $\dm_1$ on $X^0$, the result is trivial since $X^1=X^0\sqcup \dm_1(X^0)=X^0\sqcup \delta^1$ (using Def.~\ref{def:dsrdt}).
Now, assume the hypothesis is true for m-1, i.e., $X^{m-1}=\dm_{m-1} o~\dm_{m-2}~o ... o~\dm_1(X^0)=X^0\sqcup \delta^1\sqcup \delta^2 \sqcup ... \sqcup \delta^{m-1}$, then, applying the operation $\dm_m$ on $X^m$ gives:
\begin{equation*}
\begin{array}{l l l l}
X^m&=&X^{m-1}\sqcup \dm_m(X^{m-1})&\textit{(using Def.~\ref{def:dsrdt})}\\
&=&(X^0\sqcup \delta^1\sqcup ...\sqcup \delta^{m-1}) \sqcup \dm_m(X^{m-1})&\textit{(hypothesis is true for $(m-1)$)}\\
&=&X^0\sqcup \delta^1\sqcup ...\sqcup \delta^{m-1} \sqcup \dm_m(X^{m-1})&\textit{($\sqcup$ is associative)}\\
&=&X^0\sqcup \delta^1\sqcup ...\sqcup \delta^{m-1} \sqcup \delta^m &\textit{(using $\delta^m=\dm_m(X^{m-1})$)}\\
\end{array}
\end{equation*}
And the proof is complete.
\end{proof}

The above proposition means that a replica can apply multiple mutating operations, and thus producing corresponding deltas that are joined with the local replica; and then, these deltas are sent (rather than the entire object in the classical state-based CRDTs) to remote replicas, and are joined, giving the same results. In later sections, we discuss how grouping can bring further benefits once used with garbage collection.

\subsection{Decomposable \dsrdt}

Now, we introduce the decomposition concept of \dsrdt. We show that any \dsrdt object is \emph{decomposable} which can bring important performance benefits when used with anti-entropy protocols, as we explore in the following subsection.

\begin{definition}[Decomposition]
Consider a \dsrdt D=(S,M,Q), and a replica $X\in D$ with state $X_i\in S$. D is said to be decomposable if and only if there exist an arbitrary number m of states $\delta^0, \delta^1,..., \delta^m\in S$ such that $X_i=\delta^0\sqcup \delta^1\sqcup ...\sqcup \delta^m$.
\end{definition}

\begin{proposition}[Decomposable \dsrdt]
Any \dsrdt is decomposable.
\end{proposition}
\begin{proof}
As mentioned in the previous section, a \dsrdt state $X^k_i$ of replica $i$ (simply $X^k$) changes in two different ways: (1) through applying mutators in $M$, or (2) through using $join$ with other \dsrdt. Let us focus on the former point and then we show how the latter becomes easy.

First, if $X^k=\perp$ (i.e., the bottom of the semilattice $S$) then nothing to prove. Otherwise, $X^k\neq \perp$; in this case, and without loss of generality, we assume that $X^k=X^m$ is a result of causally applying an arbitrary number $m$ of $\delta$-mutators $\dm_1,\dm_2, ..., \dm_m $ on an initial state $X^0=\delta^0=\perp$ (starting from another non-bottom state is easy); then, we prove the following hypothesis by induction:
\begin{equation}
X^{m}=\delta^0\sqcup \delta^1\sqcup ...\sqcup \delta^m\textit{ where } \delta^j=\dm_j(X^{j-1})\textit{ and } 0<j\leq m.
\end{equation}
For $m=1$, meaning that only one mutator $\dm_1$ has been applied on $X^0=\delta^0$, we have $X^1=X^0\sqcup \dm_1(X^0)=\delta^0 \sqcup \delta^1$ and $\delta_1=\dm_1(X^0)$ (follows from Def.~\ref{def:dsrdt}). Then the hypothesis is true for $m=1$.

Now, suppose that the hypothesis is true for $m-1$, then it is required to prove it is correct for $m$; thus, we have the following is true:  
\begin{equation}
\label{eq:hyp_m}
X^{m-1}=\delta^0\sqcup \delta^1\sqcup ...\sqcup \delta^{m-1}\textit{ where } \delta^j=\dm_j(X^{j-1})\textit{ and } 0<j\leq m-1.
\end{equation}

Then, applying the operation $\dm_m$ on $X^{m-1}$ gives:
\begin{equation*}
\begin{array}{l l l l}
X^{m}&=&X^{m-1}\sqcup \dm_m(X^{m-1})&\textit{(using Def.~\ref{def:dsrdt})}\\
&=&(\delta^0\sqcup \delta^1\sqcup ...\sqcup \delta^{m-1}) \sqcup \dm_m(X^{m-1})&\textit{(using Eq.~\ref{eq:hyp_m})}\\
&=&\delta^0\sqcup \delta^1\sqcup ...\sqcup \delta^{m-1} \sqcup \dm_m(X^{m-1})&\textit{($\sqcup$ is associative)}\\
&=&\delta^0\sqcup \delta^1\sqcup ...\sqcup \delta^{m-1} \sqcup \delta^m &\textit{(set $\delta^m=\dm_m(X^{m-1})$)}\\
\end{array}
\end{equation*}

Thus, the proof follows for the case of applying operations.

It remains to prove that decomposition is also true once a state is joined with another state. For any two states $Y,Z \in S$, there join gives: $X=Y\sqcup Z$. And since we proved that any \dsrdt can be decomposed (by applying mutators), then, there exist an arbitrary number $m$ (resp. $n$) of $\delta$-mutators $\dm_1,\dm_2, ..., \dm_m$ (resp., $\dmm_1,\dmm_2, ..., \dmm_n$) such that: $Y=\delta^0\sqcup \delta^1\sqcup ... \sqcup \delta^m$ (resp., $Z=\delta'^0\sqcup \delta'^1\sqcup ... \sqcup \delta'^n$) where $\delta^a=\dm_a(Y^{a-1})$ and $0< a\leq m$ (resp., $\delta'^b=\dm_b(Z^{b-1})$ and $0< b\leq n$). Therefore, 
\[ X=Y\sqcup Z = (\delta^0\sqcup \delta^1\sqcup ... \sqcup \delta^m)\sqcup (\delta'^0\sqcup \delta'^1\sqcup ... \sqcup \delta'^n).\]

Therefore, $X$ is decomposable, and the proof is complete.
\end{proof}


\section{Delta Shipping of \dsrdt}
\label{sec:shipping}

We have shown in the previous section that any \dsrdt state can be decomposed into other, probably smaller, delta states. In this section, we explore how a \dsrdt can be used to improve state shipping among replicas.

\subsection{Convergence}

In this section, we show how eventual convergence is easy to achieve in \dsrdt due to their decomposable nature. For ease of presentation, we start by pairwise convergence where deltas arrive to their destination in the same sent order, and then we address the more complex issue of multiple replicas where the arrival order of deltas is not guaranteed.

\begin{proposition}[Pairwise convergence of \dsrdt]
Consider a \dsrdt D=(S,M,Q) and any two states $X_i, Y_j \in S$ of replicas i and j, respectively, such that $X_i=\delta^0\sqcup \delta^1\sqcup ... \sqcup \delta^m$ and $Y_j=\delta'^0\sqcup \delta'^1\sqcup ... \sqcup \delta'^n$, then any anti-entropy protocol (AEP) that eventually delivers all $\delta^a~\forall a$ to replica $j$ (resp., $\delta'^b~\forall b$ to replica $i$) and  joins them with $Y_j$ (resp., $X_i$), then $X$ and $Y$ eventually converge to the same state.
\end{proposition}

\begin{proof}
Since AEP eventually delivers all $\delta^a~\forall a$ to replica $j$ then, there are two cases: either (1) deltas of the same replica are delivered consecutively (i.e., grouped), or (2) deltas of both replicas are interleaved (e.g., shipped on the fly). In case (1), and without loss of generality, we assume that after an unknown timestamp $T (resp., T')$, $j$ (resp., $i$) retains $\delta^a~\forall a$ ($\delta'^b~\forall b$) in a buffer $buf_j$ ($buf_i$). Then, since AEP joins all received deltas, after a timestamp $max(T,T')$, replica $i$ (resp., $j$) joins all the deltas in $buf_i$ ($buf_j$) as follows: $X'_i=X_i\sqcup \delta'^0\sqcup \delta'^1\sqcup ... \sqcup \delta'^n$ (resp., $Y'_i=Y_i\sqcup \delta^0\sqcup \delta^1\sqcup ... \sqcup \delta^m$). Then, we proceed as follows:

\begin{equation*}
\begin{array}{l l l l}
X'_i&=&X_i\sqcup (\delta'^0\sqcup \delta'^1\sqcup ... \sqcup \delta'^n) &\textit{(using the $join$ of all deltas in $buf_i$)}\\
&=& (\delta'^0\sqcup \delta'^1\sqcup ... \sqcup \delta'^n) \sqcup X_i&\textit{($\sqcup$ is commutative and associative)}\\
&=& (\delta'^0\sqcup \delta'^1\sqcup ... \sqcup \delta'^n) \sqcup (\delta^0\sqcup \delta^1\sqcup ... \sqcup \delta^m)&\textit{(replace $X_i$)}\\
&=& Y_j \sqcup (\delta^0\sqcup \delta^1\sqcup ... \sqcup \delta^m)&\textit{(replace $Y_j$)}\\
&=& Y'_j &\textit{(using the $join$ of all deltas in $buf_j$)}\\
\end{array}
\end{equation*}
\end{proof}

In case 2, the arriving deltas are joined on the fly with the current state of the local replica, and many permutations are thus possible (e.g.,  $\delta'^0\sqcup \delta'^0\sqcup \delta^1 \sqcup \delta'^1\sqcup ... \sqcup \delta^m\sqcup ... \sqcup \delta'^n$). However, since a $join$ is always commutative and associative, simple swapping permutations can gather the deltas of each replica aside leading to a situation similar to case 1 (e.g., $\delta'^0\sqcup \delta'^1\sqcup ... \sqcup \delta'^n \sqcup \delta^0\sqcup \delta^1\sqcup ... \sqcup \delta^m$). Thus, the proof becomes close to the above one. Therefore, the two replicas converge to the same state, and the proof completes.

The above proposition does not impose any constraints on the way deltas are shipped. This is intended to leave a large margin of freedom to the designer of the anti-entropy protocol. The proof shows that convergence is achieved in both cases: sending groups of deltas and join them later on,  or immediately sending individual deltas joining them as they arrive (a la operation-based CRDTs technique). In addition, the proposition does not define the way dissemination is done. For instance, a shipping deltas can be done directly through replicas or indirectly via third party replicas. We argue that convergence is ensured in this case too, but we do not prove it, we rather introduce a more complex case where multiple replicas are exchanging their deltas.

The situation is different if multiple processes are already communicating and deltas simultaneously arrive from different replicas. This case is not trivial since a process might ship one or more merged deltas, and these deltas might have been sent by other processes.

\begin{proposition}[Multiple replicas convergence of \dsrdt]
Consider a \dsrdt D=(S,M,Q) and an object $X\in D$ distributed on $n$ replicas. Each replica i has a state $X_i$ of $X$ that is decomposable into $a_i-b_i+1$ deltas: $\delta_i^{a_i}, \delta_i^{a_i+1}, ..\delta_i^{b_i}$. Any anti-entropy protocol (AEP) that eventually delivers and joins all $\delta_i^x~\forall x$ to all other replicas $X_k~\forall k\neq i$, then all replicas of X eventually converge to the same state.
\end{proposition}

\begin{proof}
 Suppose that, initially, $X_i=X^\perp$ for any process $p_i~ \forall i\leq n$; then process $p_i$ ships $a_i-b_i+1$ deltas: $\delta_i^{a_i}, \delta_i^{a_i+1}, ..\delta_i^{b_i}$ to all other processes. Since AEP eventually delivers all deltas to every other process (either directly or indirectly), then there exist an unknown instant $T$ such that all process receive $\delta_i^{a_i}, \delta_i^{a_i+1}, ..\delta_i^{b_i}~\forall i\leq n$. Since deltas received from a single process $p_t$ are not guaranteed to be causally ordered, this is also true for deltas received from distinct replicas. Therefore, at instant $T$, every process must have received and joined all deltas from different processes, probably, in a different random order, we denote this by the following join permutation: 
\begin{equation*}
X'_i=X^\perp \sqcup \mathsf{rand}(\bigsqcup_{1\leq x\leq n}^{a_x\leq z\leq b_x} \delta_x^z)
\end{equation*}

Then, since $join$ is commutative, we can reorder the above join permutation using the following recursive steps on $X'_i$:
\begin{itemize}
\item Step 1 ($lookup$): from $a=1$ to $n$, search (from left to right) for the first occurrence of $\delta_a$ in $X'_i$, call it $\delta_a^{current}$.
\item Step 2 ($swap$): go from $\delta_a^{current}$ backwards in $X'_i$, and compare possible pairs: $\delta_b^z\sqcup \delta_a^{current}$, if $a<b$ then swap the order to $\delta_a^{current}\sqcup \delta_b^z$ (this possible since $\sqcup$ is commutative).
\item Step 3 ($iterate$): if $b<a$, go to Step 1; otherwise go to Step 2. 
\end{itemize}

By the end of this reordering, we get a new ordered state $X'_i$ as follows:
\begin{equation*}
X'_i=X^\perp \sqcup \left(\bigsqcup_{a_1\leq k\leq b_1} \delta_1^{k}\right) \sqcup
\left(\bigsqcup_{a_2\leq k\leq b_2} \delta_2^{k}\right) \sqcup ... \sqcup 
\left(\bigsqcup_{a_n\leq k\leq b_n} \delta_n^{k}\right)
\end{equation*}

Since this permutation is independent from $i$, and all processes received the same deltas, they will have the same permutation as $X'_i$; and thus $X$ will be consistent on all processes, and the proof completes.

Notice that we did not consider the cases of multiple shipping (if third party process shipped deltas from another process) since $\sqcup$ is idempotent and thus joining the same deltas which were already joined (probably through another channel or third party replica) will have no impact on the final state, as soon as they are all eventually delivered as ensured by AEP.
\end{proof}

\subsection{Redundant Shipping of \dsrdt}
In this section, we study the \emph{redundant payload shipping} of \dsrdt which we define as the shipping overhead of a part of an object payload (or the entire object) which was already shipped. We show how, using \dsrdt, we can significantly reduce the overhead of shipping in state-based CRDTs by avoiding shipping redundant information. 

\begin{proposition}[Redundant payload shipping of \dsrdt vs. CRDT]
The redundant payload shipping of a replica payload of a \dsrdt is less than or equal to that of a corresponding state-based CRDT.
\end{proposition}
\begin{proof}
Since any state-based CRDT is a \dsrdt where all $\delta$-mutators are \emph{maximal} (see Subsection~\ref{subs:dsrdt}) then the equivalence is true. 

On the other hand, if there exist at least one $\delta$-mutator that is not maximal, then, at some instant $T$, there exist at least one delta $\delta^k=\dm_k$ such that the state on a certain replica $i$: $X_i^k=\delta^0\sqcup \delta^1\sqcup ... \sqcup \delta^k$ and $size(\dm_k(X_i^{k-1}))<size(m(X_i^{k-1}))=size(X_i^k)$. But according to the state transition methods in Subsection~\ref{subs:transition}, a \dsrdt replica only ships $\delta^k$ to other replicas, whereas in classical state-based CRDTs $X_i^k$ will be shipped. Thus, the redundant payload shipping of the CRDT induced by replica $i$ will be greater than that of the corresponding \dsrdt by:   $size(m(X_i^{k-1})) - size(\dm_k(X_i^{k-1}))>0$; and the proof completes.

\end{proof}

Now we continue by defining \emph{granularity}, and then we show how it can impact the shipping overhead.

\begin{definition}[Granularity]
Consider a \dsrdt D=(S,M,Q), and a replica $X\in S$ with state $X_i^m=\delta^0\sqcup \delta^1\sqcup ...\sqcup \delta^m,~\forall m$. $X_i^m$ is said to be 'fine-grained' if and only if $\forall \delta^j, \exists \dm_j\in M$ such that: $\delta^j=\dm_j(X_i^j),~\forall j\leq m$ and $\dm_i$ is 'minimal'. Otherwise, we say that $X_i^m$ is 'coarse-grained'. 
\end{definition}

\begin{proposition}[Redundant payload shipping of fine-grained \dsrdt]
No \dsrdt redundant payload shipping lower than that of a fine-grained \dsrdt can be achieved.
\end{proposition}
\begin{proof}
Suppose that there exist a payload shipping overhead of a coarse-grained replica $X\in S$ of a \dsrdt D=(S,M,Q) lower than that of a fine-grained \dsrdt of equivalent state $X'\in S$. If $X_i^{'k}=\delta^0\sqcup \delta^1\sqcup ... \sqcup \delta^{k'}\sqcup ... \sqcup \delta^m$, then there exist at least one $\delta$-mutator $\dm_k$ and corresponding $\delta^k$ in a replica state $X_i^k=\delta^0\sqcup \delta^1\sqcup ... \sqcup \delta^k\sqcup ... \sqcup \delta^m$ such that $\delta^{k'}>\delta^k=\dm_k(X^{k-1})$. But since $X'$ is fine-grained and $X^{k-1}=X^{'k'-1}$, then there exist a minimal $\delta$-mutator $\dm_{k'}$ such that $\delta^{k'}=\dm_{k'}(X^{k-1})$; but $\delta^{k'}>\delta^k=\dm_k(X^{k-1})$, thus $\dm_{k'}(X^{k-1})>\dm_k(X^{k-1})$; this means that $\dm_{k'}$ is not minimal. This contradicts with the assumption that $X'$ is fine-grained and, thus, the proof completes.
\end{proof}

\subsection{Shipping Delta-groups}
In the previous sections, we have shown that convergence can be achieved if the used anti-entropy protocol ensures that all deltas are delivered to all replicas without delving into details of shipping. In fact, sometimes batching deltas via sending delta-groups can reduce the overhead of shipping and joining. 

In practice, depending on the design choices, batching messages can bring many benefits in communication systems especially whenever message headers and kernel calls are costly. However, \dsrdt has an additional interesting property that makes batching, i.e., shipping delta-groups, more efficient under some circumstances, which reduces the shipping overhead.

In principle, this is not always true. Since the states of a \dsrdt form a semilattice, then applying new operations or \emph{joins} always increment the state size. However, once garbage collection (GC) is used, as in~\cite{garbage collection}, the shipping overhead of delta groups of a \dsrdt can be lower than that of shipping individual deltas gradually. For instance, multiple \emph{adds} and then \emph{removes} of the same items in a \emph{Set} of a single replica are not shipped to other replicas if GC is used before shipping. The intuition is that the \emph{removes} will cancel the effect of the \emph{adds}, and thus neither the items nor the tombstones will be shipped.

This fact, however, does not hold true for datatypes that are only incremental in terms of state size, .e.g, add-only counter and grow-only set. The reason is that garbage collection itself has no effect on the state size in these datatypes, and thus, shipping delta-groups has no $\delta$-SRDT-specific advantages over sending individual deltas (expect those related to headers and kernel calls). 


==> mathdefs.tex <==
\RequirePackage{latexsym}
\RequirePackage{dsfont}



\mathcode`.="613A
\mathcode`|="326A

\let\es=\relax


\newcommand\tx[1]{\hbox{ #1 }}
\newcommand{\defeq}{\stackrel{.}{=}}

\let\vect=\overrightarrow
\let\iff=\Leftrightarrow
\let\implies=\Rightarrow
\let\implied=\Leftarrow

\let\sqleq=\sqsubseteq
\let\sqgeq=\sqsupseteq
\let\pleq=\sqleq
\let\pgeq=\sqgeq

\def\land{\mathrel{\wedge}}
\def\lor{\mathrel{\vee}}
\let\bigland=\bigwedge
\let\biglor=\bigvee

\def\preleq{\mathrel{
  \raise 2pt\hbox{$\mathop\sqsubset\limits_{\hbox{$\sim$}}$}%
}}


\let\union=\cup
\let\bigunion=\bigcup
\let\join=\sqcup
\let\bigjoin=\bigsqcup
\let\meet=\sqcap
\newcommand{\down}{\mathord{\downarrow}}

\newcommand\setsize[1]{\left| #1 \right|}
\newcommand\domxtn{\mathbin{\stackrel{+}{|}}}
\newcommand\domainsub{\mathop{\lhd\mkern-14mu-}}


\newcommand{\map}{\mathrel{\hookrightarrow}}
\newcommand\goesto[1]{{\mathop{\longrightarrow}\limits^{#1}}}
\newcommand\goes{\longrightarrow}


\newcommand\auxfun[1]{\expandafter\newcommand\csname #1\endcsname{%
 \mathop{\hbox{$\mathsf{#1}$}}\nolimits}}
 \newcommand\af[1]{\mathop{\hbox{$\mathsf{#1}$}}\nolimits}
 \newcommand\kw[1]{\mathrel{\hbox{$\mathbf{#1}$}}}

\auxfun{Max}
\auxfun{fix}
\auxfun{dom}
\auxfun{fst}
\auxfun{snd}
\auxfun{ran}


\newcommand{\pow}[1]{{\cal P}(#1)}
\newcommand{\bool}{\mathds{B}}
\newcommand{\nat}{\mathds{N}}
\newcommand{\ids}{\mathds{I}}




\newcommand\letin[2]{\mathop{\hbox{$\mathrm{let}$}} #1 \Leftarrow #2 . }
\newcommand\lift[1]{\lfloor #1 \rfloor}

\newcommand\true{\mathrm{true}}
\newcommand\false{\mathrm{false}}


\newcommand\iffdef{\mathrel{\Longleftrightarrow}}
\newcommand\nullstring{\epsilon}
\newcommand\pfunc{\hookrightarrow}
\newcommand\func{\rightarrow}


